Statistical Analysis of the LMS Algorithm for Proper and Improper Gaussian Processes

The LMS algorithm is one of the most widely used techniques in adaptive filtering. Accurate modeling of the algorithm in various circumstances is paramount to achieving an efficient adaptive Wiener filter design process. In the recent decades, concerns have been raised on studying improper signals and providing an accurate model of the LMS algorithm for both proper and improper signals. Other models for the LMS algorithm for improper signals available in the scientific literature either make use of the independence assumptions regarding the desired signal and the input signal vector, or are exclusive to proper signals; it is shown that by not considering these assumptions a more general model can be derived. In the presented simulations it is possible to verify that the model introduced in this paper outperforms the other available models.

==> chapters/sa.tex <==
% https://www.latex-tutorial.com/tutorials/lists/
\subsection{Simplifying Assumptions}
For mathematical tractability, the analysis is performed under the following set of simplifying assumptions:
\begin{description}
\item[A1]$\mathbf{x}(n)$ and $\mathit{{d(n)}}$ are zero-mean complex-valued Gaussian random processes;
\item[A2]$\mathit{{m(n)}}$ is a zero-mean complex-valued white Gaussian random process, which is statistically independent of any other aleatory signal;    
\item[A3]The statistical dependence between $\mathbf{w}(n-1)$ and $\mathbf{x}(n)$ can be neglected.
%\item[A4]Matrix $\mathbf{R_e}$ is positive-definite.
\end{description}

\subsection{Mean Weight Vector Behavior}
Taking unconditional expectation on both sides of (\ref{eqn:w_update}), and using the above simplifying assumptions, leads to the recursive equation for the transient behavior of $E\{\mathbf{w}(n)\}$:
\begin{equation}
     E\{\mathbf{w}(n)\}=[\mathbf{I}-\mu\mathbf{R}]E\{\mathbf{w}(n-1)\}+ \mu\mathbf{p} \label{eqn:Ew_update}   
\end{equation}
where $\mathbf{I}$ denotes an $\mathit{N}$-by-$\mathit{N}$ identity matrix. \par
The steady state behavior of $E\{\mathbf{w}(n)\}$ can be obtained from (\ref{eqn:Ew_update}), assuming that the LMS algorithm converges when $n\to\infty$:
\begin{equation} \label{eqn:w_infty}
\begin{split}
     \mathbf{w_{\infty}}& \triangleq \lim_{n\to\infty} E\{\mathbf{w}(n)\}   
     \\&=\mathbf{R}^{-1}\mathbf{p} 
\end{split}
\end{equation}
This means that the LMS algorithm converges to the optimum solution in (\ref{eqn:wo}), being the minimum MSE given by (\ref{eqn:MMSE}).

\subsection{Mean Weight Error Vector Behavior}
% SUGESTÃO PARA ESCREVER "N por 1" ==> $N \times 1$
Defining the $\mathit{N}$-by-1 weight error vector at instant $\mathit{n}$:
\begin{equation}
    \mathbf{v}(n) \triangleq \mathbf{w}(n) - \mathbf{w_{\infty}}
    \label{eqn:Weight_error}   
\end{equation}
from (\ref{eqn:w_update}), yields
\begin{equation}
     \mathbf{v}(n)=\mathbf{v}(n-1)+\mu e^*(n) \mathbf{x}(n) \label{eqn:v_update}   
\end{equation}
Taking unconditional expectation of (\ref{eqn:v_update}), under the simplifying assumptions again, leads to 
\begin{equation}
\begin{split}
    E\{\mathbf{v}(n)\}&=[\mathbf{I}-\mu\mathbf{R}]E\{\mathbf{v}(n-1)\} \\ &=[\mathbf{I}-\mu\mathbf{R}]^{n}E\{\mathbf{v}(0)\} \label{eqn:Ev_update}    
\end{split}
\end{equation}
Hence, convergence in the mean of $\mathbf{w}(n)$ requires all the eigenvalues of $\mathbf{I}-\mu\mathbf{R}$ to be inside the unit circle. In this case, the solution  $\mathbf{w}(n)$ becomes unbiased as $n\to\infty$. Now, using the orthogonal eigendecomposition $\mathbf{R}=\mathbf{Q \Lambda Q}^H$, where $\mathbf{\Lambda}=diag[\lambda_1,\lambda_2,...,\lambda_N]$ is the diagonal matrix with the eigenvalues of $\mathbf{R}$, and $\mathbf{Q}$ is the unitary matrix consisting of the associated eigenvectors ($\mathbf{QQ^{\mathit{H}}}=\mathbf{I}$), (\ref{eqn:Ev_update}) yields
\begin{equation}
    E\{\mathbf{v}(n)\}=\mathbf{Q}[\mathbf{I}-\mu\mathbf{\Lambda}]^{n}\mathbf{Q}^HE\{\mathbf{v}(0)\} \label{eqn:EigenEv_update}
\end{equation}
From (\ref{eqn:EigenEv_update}), an upper limit for $\mu$ ensuring the convergence of the LMS algorithm can be determined:
\begin{equation}
    0<\mu\ll\frac{1}{\lambda_{max}}   
\end{equation}
where $\lambda_{max}$ is the largest eigenvalue of $\mathbf{R}$, or
\begin{equation} \label{eqn:mi_limit}
    0<\mu<\frac{1}{tr[\mathbf{R}]}
\end{equation}
with $tr[\mathbf{R}]=\sum_{i=1}^N\lambda_i$, and $tr[\bullet]$ denoting the trace of a square matrix $\bullet$.
The time constant of each convergence natural mode is
\begin{equation} \label{eqn:mi_limit}
    \tau_i=\frac{1}{ln(1-\mu\lambda_i)}   
\end{equation}
for $\mathit{i}=1, 2,...,N$. Then, for $\mu\lambda_i\ll1$,
\begin{equation} \label{eqn:mi_limit}
    \tau_i\approx\frac{1}{\mu\lambda_i}   
\end{equation}
So, the behavior of the mean weight error vector is dictated only by the eigenvalues of $\mathbf{R}$, regardless of whether $\mathbf{x}(n)$ is proper or improper.

\subsection{Mean Square Error Behavior}
From (\ref{eqn:error_signal}) and (\ref{eqn:Weight_error}), under the simplifying assumptions once again, taking first the conditional expectation, for a given $\mathbf{v}(n-1)$, and after by averaging over $\mathbf{v}(n-1)$, leads to
\begin{equation} \label{eqn:MSE_update}
\begin{split}
    J(\mathit{n})&=E\{|e(n)|^2\}
    \\&=J_{min}+J_{ex}(\mathit{n})
\end{split}
\end{equation}
where $\mathit{J_{min}}$ is the minimum MSE in (\ref{eqn:MMSE}),
\begin{equation} \label{eq:Jex}    J_{ex}(\mathit{n})=tr[\mathbf{R}\mathbf{V}(n-1)]
\end{equation}
accounts for the excess MSE at time $\mathit{n}$ of the stochastic gradient-based adaptation technique, and
\begin{equation} \label{eq:V(n-1)}
\mathbf{V}(n-1)=E\{\mathbf{v}(n-1)\mathbf{v^{\mathit{H}}}(n-1)\}
\end{equation}
is the weight error correlation matrix.

\subsection{Excess MSE}
From (\ref{eqn:v_update}) and (\ref{eq:V(n-1)}), yields
\begin{equation} \label{eq:V_update}
\mathbf{V}(n-1)=\mathbf{V}(n-2)+\mu[\mathbf{A}(n-1)+\mathbf{A}^{\mathit{H}}(n-1)]+\mu^{2}\mathbf{B}(n-1)
\end{equation}
where
\begin{equation} \label{eq:A(n-1)}
\mathbf{A}(n-1)=E\{\mathbf{v}(n-2)\mathbf{x^{\mathit{H}}}(n-1)e(n-1)\}
\end{equation}
and
\begin{equation} \label{eq:B(n-1)}
\mathbf{B}(n-1)=E\{\mathbf{x}(n-1)\mathbf{x^{\mathit{H}}}(n-1)e(n-1)e^*(n-1)\}
\end{equation}
From (\ref{eqn:error_signal}) and (\ref{eqn:Weight_error}), based on A1-A3, follows that
\begin{equation} \label{eq:A_update}
\mathbf{A}(n-1)=-\mathbf{V}(n-2)\mathbf{R}
\end{equation}
Under A1 and A2, the fourth-order moment in (\ref{eq:B(n-1)}) can be obtained based on the Gaussian moment-factoring theorem. It can be rewritten as
\begin{equation} \label{eq:B_update}
%%\begin{split}
   \mathbf{B}(n-1)=J(\mathit{n}-1)\mathbf{R}+\mathbf{U}(n-1)+\mathbf{S}(n-1)\\
%%   &+\mathbf{u}(n-1)\mathbf{u^{\mathit{H}}}(n-1)+\\
%%   &+\mathbf{s}(n-1)\mathbf{s^{\mathit{H}}}(n-1)
%%\end{split}
\end{equation}
where
\begin{equation} \label{eq:J(n-1)}
J(\mathit{n}-1)=E\{|e(n-1)|^2\}
\end{equation}
\begin{equation}
   \mathbf{U}(n-1)=
E\{\mathbf{x}(n-1)e^*(n-1)\}E\{e(n-1)\mathbf{x^{\mathit{H}}}(n-1)\}
\end{equation}
and
\begin{equation}
\mathbf{S}(n-1)=
E\{\mathbf{x}(n-1)e(n-1)\}E\{e^*(n-1)\mathbf{x^{\mathit{H}}}(n-1)\}
\end{equation}
Using A1-A3, (\ref{eqn:error_signal}) and (\ref{eqn:Weight_error}), yields
\begin{equation} \label{eq:U(n-1)}
\mathbf{U}(n-1)=\mathbf{R}\mathbf{V}(n-2)\mathbf{R}
\end{equation}
Now, taking into account that $\mathbf{x}(n)$, $\mathit{{d(n)}}$  and $\mathit{{m(n)}}$ are improper processes, leads to
\begin{equation} \label{eq:S(n-1)}
\begin{split}
\mathbf{S}(n-1)=&\mathbf{k}\mathbf{k^{\mathit{H}}}-\mathbf{k}E\{\mathbf{v}^{\mathit{T}}(n-2)\}\mathbf{C}^{\mathit{H}}\\
&-\mathbf{C}E\{\mathbf{v}^*(n-2)\}\mathbf{k^{\mathit{H}}}+\mathbf{C}\mathbf{V}^*(n-2)\mathbf{C}^{\mathit{H}}
\end{split}
\end{equation}
where
\begin{equation} \label{eq:k}
\mathbf{k}=\mathbf{q}-\mathbf{C}\mathbf{w^*_{\infty}}
\end{equation}
is the pseudo-cross-correlation vector  between $\mathbf{x}(n)$ and $\mathit{e_o(n)}$ in (\ref{eqn:Exeo}).
Equations (\ref{eq:S(n-1)}), (\ref{eq:U(n-1)}), (\ref{eq:B_update}), (\ref{eq:A_update}), (\ref{eq:V_update}) and (\ref{eq:Jex}) resume the recursive expression for updating $J_{ex}(\mathit{n})$ and, consequently, the MSE behavior in (\ref{eqn:MSE_update}). \par
The steady-state MSE is reached after algorithm converge, being define as
\begin{equation} \label{eq:J_infinite}
   J_{\infty} \triangleq \lim_{n\to\infty} J(\mathit{n}) = J_{min}+J_{ex}(\infty)
\end{equation}
where
\begin{equation}
J_{ex}(\infty)\triangleq \lim_{n\to\infty}J_{ex}(n)=tr[\mathbf{R}\mathbf{V}_\infty]
\end{equation}
and
\begin{equation}
\mathbf{V}_\infty \triangleq \lim_{n\to\infty} \mathbf{V}(n-1)
\end{equation}
From (\ref{eq:V_update}), (\ref{eq:A_update}) and (\ref{eq:B_update}), it can be shown that
\begin{equation}
tr[\mathbf{R}\mathbf{V}_\infty]=\frac{\mu}{2}(J_{\infty}tr[\mathbf{R}]+tr[\mathbf{s}_\infty\mathbf{s_\infty^{\mathit{H}}}])
\end{equation}
and
\begin{equation}
J_{ex}(\infty)=\frac{{\mu}(J_{min}tr[\mathbf{R}]+tr[\mathbf{s}_\infty\mathbf{s_\infty^{\mathit{H}}}])}{2-{\mu}tr[\mathbf{R}]}
\end{equation}

\begin{equation}
\mathbf{s}_\infty \triangleq \lim_{n\to\infty} \mathbf{s}(n-1)=\mathbf{q}-\mathbf{C}\mathbf{w^*_{\infty}}
\end{equation}
Finally, solving for $J_{\infty}$ yields
\begin{equation}
J_{\infty}=J_{min}\left(1+ \frac{{\mu}tr[\mathbf{R}]}{2-{\mu}tr[\mathbf{R}]}\right)+\frac{{\mu}tr[\mathbf{s}_\infty\mathbf{s_\infty^{\mathit{H}}}])}{2-{\mu}tr[\mathbf{R}]}
\end{equation}
\subsection{Misadjustment}
When (\ref{eqn:mi_limit}) holds, the misadjustment for the LMS algorithm is given by
\begin{equation} \label{eqn:xi}
%\begin{split}
\xi=\frac{J_{ex}(\infty)}{J_{min}}
=\frac{{\mu}(tr[\mathbf{R}]+tr[\mathbf{s}_\infty\mathbf{s_\infty^{\mathit{H}}}]/J_{min})}{2-{\mu}tr[\mathbf{R}]}
%\end{split}
\end{equation}
For a sufficiently small $\mu$, this results in
\begin{equation}
\xi \approx \frac{1}{2}{\mu}(tr[\mathbf{R}]+tr[\mathbf{s}_\infty\mathbf{s_\infty^{\mathit{H}}}]/J_{min})
\end{equation}
which means that increasing $\mu$ increases the misadjustment.
From (\ref{eqn:xi}), a stability upper bound can also be established for $\mu$:
\begin{equation}
\mu_{max}=\frac{2}{tr[\mathbf{R}]}
\end{equation}
